An action language-based formalisation of an abstract argumentation framework

An abstract argumentation framework is a commonly used formalism to provide a static representation of a dialogue. However, the order of enunciation of the arguments in an argumentative dialogue is very important and can affect the outcome of this dialogue. In this paper, we propose a new framework for modelling abstract argumentation graphs, a model that incorporates the order of enunciation of arguments. By taking this order into account, we have the means to deduce a unique outcome for each dialogue, called an extension. We also establish several properties, such as termination and correctness, and discuss two notions of completeness. In particular, we propose a modification of the previous transformation based on a "last enunciated last updated" strategy, which verifies the second form of completeness.

==> fig_exemple_fin.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp32394197299921523] 
\draw  [line width=0.75]  (38.8,251.2) -- (74.6,251.2) -- (74.6,270.54) -- (38.8,270.54) -- cycle ;
%Straight Lines [id:da5103454315814933] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (85.53,6.3) -- (84.6,299.8) ;
%Straight Lines [id:da9625799604219181] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (181.03,5.8) -- (181.8,299.8) ;
%Straight Lines [id:da937826652519754] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (286.6,5.8) -- (285.8,299.4) ;
%Shape: Rectangle [id:dp39055029505322625] 
\draw  [line width=0.75]  (133.09,41.57) -- (168.89,41.57) -- (168.89,60.91) -- (133.09,60.91) -- cycle ;
%Shape: Polygon [id:dp25831662543105294] 
\draw   (27.7,21.73) -- (21,33.26) -- (7.6,33.26) -- (0.91,21.73) -- (7.6,10.19) -- (21,10.19) -- cycle ;
%Shape: Polygon [id:dp17264867524000027] 
\draw   (121.4,21.73) -- (114.7,33.26) -- (101.3,33.26) -- (94.6,21.73) -- (101.3,10.19) -- (114.7,10.19) -- cycle ;
%Shape: Polygon [id:dp9933858680624272] 
\draw   (215.4,23.23) -- (208.7,34.76) -- (195.3,34.76) -- (188.6,23.23) -- (195.3,11.69) -- (208.7,11.69) -- cycle ;
%Shape: Rectangle [id:dp8416513794122603] 
\draw  [line width=0.75]  (236.69,189.97) -- (272.49,189.97) -- (272.49,209.31) -- (236.69,209.31) -- cycle ;
%Curve Lines [id:da03689428077806867] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (74.74,260.46) .. controls (110.24,284.75) and (154.9,290.88) .. (187.62,260.92) ;
\draw [shift={(188.6,260)}, rotate = 136.62] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da9511759619364188] 
\draw    (74.74,260.46) .. controls (94.3,224.74) and (104.69,262.24) .. (131.75,231.26) ;
\draw [shift={(133,229.8)}, rotate = 129.81] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Shape: Regular Polygon [id:dp0962459706720944] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (215.1,52.33) -- (208.41,63.92) -- (195.03,63.92) -- (188.34,52.33) -- (195.03,40.75) -- (208.41,40.75) -- cycle ;
%Curve Lines [id:da23781812589748064] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (74.74,260.46) .. controls (136.15,295.88) and (173.1,260.09) .. (189.61,238.31) ;
\draw [shift={(190.6,237)}, rotate = 126.53] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Shape: Regular Polygon [id:dp5863365292722718] 
\draw   (27.78,51.53) -- (21.09,63.12) -- (7.71,63.12) -- (1.02,51.53) -- (7.71,39.95) -- (21.09,39.95) -- cycle ;
%Shape: Polygon [id:dp668166576601705] 
\draw   (27.4,81.13) -- (20.7,92.66) -- (7.3,92.66) -- (0.6,81.13) -- (7.3,69.59) -- (20.7,69.59) -- cycle ;
%Shape: Regular Polygon [id:dp1615790376024172] 
\draw   (27.48,110.93) -- (20.79,122.52) -- (7.41,122.52) -- (0.72,110.93) -- (7.41,99.35) -- (20.79,99.35) -- cycle ;
%Shape: Polygon [id:dp5652109778432169] 
\draw   (27.8,140.73) -- (21.1,152.26) -- (7.7,152.26) -- (1,140.73) -- (7.7,129.19) -- (21.1,129.19) -- cycle ;
%Shape: Regular Polygon [id:dp5554624960747061] 
\draw   (27.88,170.53) -- (21.19,182.12) -- (7.81,182.12) -- (1.12,170.53) -- (7.81,158.95) -- (21.19,158.95) -- cycle ;
%Shape: Regular Polygon [id:dp13320010668351145] 
\draw   (27.48,229.53) -- (20.79,241.12) -- (7.41,241.12) -- (0.72,229.53) -- (7.41,217.95) -- (20.79,217.95) -- cycle ;
%Shape: Regular Polygon [id:dp33133807114366276] 
\draw   (121.78,51.8) -- (115.09,63.39) -- (101.71,63.39) -- (95.02,51.8) -- (101.71,40.22) -- (115.09,40.22) -- cycle ;
%Shape: Polygon [id:dp7206917082119544] 
\draw   (121.4,81.4) -- (114.7,92.94) -- (101.3,92.94) -- (94.6,81.4) -- (101.3,69.86) -- (114.7,69.86) -- cycle ;
%Shape: Regular Polygon [id:dp689513993897114] 
\draw   (121.48,111.2) -- (114.79,122.79) -- (101.41,122.79) -- (94.72,111.2) -- (101.41,99.62) -- (114.79,99.62) -- cycle ;
%Shape: Polygon [id:dp3553082836345921] 
\draw   (121.8,141) -- (115.1,152.54) -- (101.7,152.54) -- (95,141) -- (101.7,129.46) -- (115.1,129.46) -- cycle ;
%Shape: Regular Polygon [id:dp08808706934177946] 
\draw   (121.88,170.8) -- (115.19,182.39) -- (101.81,182.39) -- (95.12,170.8) -- (101.81,159.22) -- (115.19,159.22) -- cycle ;
%Shape: Regular Polygon [id:dp3825724531298007] 
\draw   (121.48,229.8) -- (114.79,241.39) -- (101.41,241.39) -- (94.72,229.8) -- (101.41,218.22) -- (114.79,218.22) -- cycle ;
%Shape: Polygon [id:dp6015095613297166] 
\draw   (121.4,259) -- (114.7,270.54) -- (101.3,270.54) -- (94.6,259) -- (101.3,247.46) -- (114.7,247.46) -- cycle ;
%Shape: Polygon [id:dp9730868685192309] 
\draw   (215.4,82.4) -- (208.7,93.94) -- (195.3,93.94) -- (188.6,82.4) -- (195.3,70.86) -- (208.7,70.86) -- cycle ;
%Shape: Regular Polygon [id:dp04394747212171679] 
\draw   (215.48,112.2) -- (208.79,123.79) -- (195.41,123.79) -- (188.72,112.2) -- (195.41,100.62) -- (208.79,100.62) -- cycle ;
%Shape: Polygon [id:dp625486130912703] 
\draw   (215.8,142) -- (209.1,153.54) -- (195.7,153.54) -- (189,142) -- (195.7,130.46) -- (209.1,130.46) -- cycle ;
%Shape: Regular Polygon [id:dp6973070301209515] 
\draw   (215.88,171.8) -- (209.19,183.39) -- (195.81,183.39) -- (189.12,171.8) -- (195.81,160.22) -- (209.19,160.22) -- cycle ;
%Shape: Polygon [id:dp15730100429007365] 
\draw   (215.4,260) -- (208.7,271.54) -- (195.3,271.54) -- (188.6,260) -- (195.3,248.46) -- (208.7,248.46) -- cycle ;
%Shape: Polygon [id:dp7669928381847199] 
\draw   (324.4,81.4) -- (317.7,92.94) -- (304.3,92.94) -- (297.6,81.4) -- (304.3,69.86) -- (317.7,69.86) -- cycle ;
%Shape: Regular Polygon [id:dp8720689089102229] 
\draw   (324.48,111.2) -- (317.79,122.79) -- (304.41,122.79) -- (297.72,111.2) -- (304.41,99.62) -- (317.79,99.62) -- cycle ;
%Shape: Polygon [id:dp8686588781646976] 
\draw   (324.8,141) -- (318.1,152.54) -- (304.7,152.54) -- (298,141) -- (304.7,129.46) -- (318.1,129.46) -- cycle ;
%Shape: Regular Polygon [id:dp58257999600958] 
\draw   (324.88,170.8) -- (318.19,182.39) -- (304.81,182.39) -- (298.12,170.8) -- (304.81,159.22) -- (318.19,159.22) -- cycle ;
%Shape: Polygon [id:dp5246042913035425] 
\draw   (324.4,200) -- (317.7,211.54) -- (304.3,211.54) -- (297.6,200) -- (304.3,188.46) -- (317.7,188.46) -- cycle ;
%Shape: Polygon [id:dp40275693353577746] 
\draw   (324.4,259) -- (317.7,270.54) -- (304.3,270.54) -- (297.6,259) -- (304.3,247.46) -- (317.7,247.46) -- cycle ;
%Shape: Rectangle [id:dp294546304037402] 
\draw  [line width=0.75]  (133.09,220.57) -- (168.89,220.57) -- (168.89,239.91) -- (133.09,239.91) -- cycle ;
%Shape: Regular Polygon [id:dp13124017670187849] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (323.1,52.33) -- (316.41,63.92) -- (303.03,63.92) -- (296.34,52.33) -- (303.03,40.75) -- (316.41,40.75) -- cycle ;
%Shape: Regular Polygon [id:dp6955758409780655] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (215.1,230.33) -- (208.41,241.92) -- (195.03,241.92) -- (188.34,230.33) -- (195.03,218.75) -- (208.41,218.75) -- cycle ;
%Shape: Regular Polygon [id:dp41515587858602165] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (324.1,230.33) -- (317.41,241.92) -- (304.03,241.92) -- (297.34,230.33) -- (304.03,218.75) -- (317.41,218.75) -- cycle ;
%Curve Lines [id:da9290568647401355] 
\draw    (74.74,260.46) .. controls (87.4,89) and (131.4,305) .. (133.09,60.91) ;
\draw [shift={(133.09,60.91)}, rotate = 90.4] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da0024038948177537156] 
\draw    (74.74,260.46) .. controls (90.92,188.96) and (147.23,207.61) .. (235.66,195.98) ;
\draw [shift={(237,195.8)}, rotate = 172.34] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da9423544130706317] 
\draw    (169.14,230.06) .. controls (176.09,204.98) and (193.66,205.77) .. (235.09,203.12) ;
\draw [shift={(237,203)}, rotate = 176.26] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da07687685155568191] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (74.74,260.46) .. controls (88.13,300.8) and (222.84,295.45) .. (296.5,259.54) ;
\draw [shift={(297.6,259)}, rotate = 153.62] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da17080960388415456] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (74.74,260.46) .. controls (88.36,259.78) and (80.46,259.9) .. (92.73,259.12) ;
\draw [shift={(94.6,259)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da6369256315030506] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (169,52.78) .. controls (182.62,52.1) and (174.24,53.15) .. (186.47,52.44) ;
\draw [shift={(188.34,52.33)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da5460890529535121] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (169.14,230.06) .. controls (182.76,229.38) and (174.38,230.43) .. (186.61,229.73) ;
\draw [shift={(188.48,229.62)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da9866128326016497] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (169.14,230.06) .. controls (187.91,203.01) and (256.5,224.73) .. (295.58,230.1) ;
\draw [shift={(297.34,230.33)}, rotate = 187.26] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da3372282256776671] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (169,52.78) .. controls (193.95,17.75) and (250.26,58.57) .. (294.99,52.53) ;
\draw [shift={(296.34,52.33)}, rotate = 171.06] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da7931620072938754] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (273.22,200.11) .. controls (286.84,199.43) and (283.06,200.78) .. (295.7,200.11) ;
\draw [shift={(297.6,200)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da3170103066051301] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (74.74,260.46) .. controls (118.16,315.64) and (262.47,264.45) .. (298.73,238.19) ;
\draw [shift={(299.8,237.4)}, rotate = 142.92] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da2974445519606693] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (74.74,260.46) .. controls (87.54,158.68) and (268.35,187.37) .. (299.3,193.08) ;
\draw [shift={(301,193.4)}, rotate = 190.78] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da007173676928789563] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (74.74,260.46) .. controls (87.8,155) and (157.8,229.8) .. (191.4,58.6) ;
\draw [shift={(191.4,58.6)}, rotate = 101.1] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da8424571147503932] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (74.74,260.46) .. controls (81.4,151.4) and (260.2,192.6) .. (299.4,57.8) ;
\draw [shift={(299.4,57.8)}, rotate = 106.21] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da832051990599513] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (169.14,230.06) .. controls (184.45,192.58) and (255.95,229.84) .. (299.3,206.91) ;
\draw [shift={(300.6,206.2)}, rotate = 150.54] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Shape: Polygon [id:dp822443066516893] 
\draw   (322.8,22.63) -- (316.1,34.16) -- (302.7,34.16) -- (296,22.63) -- (302.7,11.09) -- (316.1,11.09) -- cycle ;

% Text Node
\draw (27.13,289.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$t=28$};
% Text Node
\draw (44,257.6) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$enu_{n}$};
% Text Node
\draw (133.09,47.97) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$una_{n,c}$};
% Text Node
\draw (116.67,290.33) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$t=29$};
% Text Node
\draw (215.8,289.9) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$t=30$};
% Text Node
\draw (301,288.9) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$t=31$};
% Text Node
\draw (14.3,22.73) node  [font=\small]  {$b$};
% Text Node
\draw (108,22.73) node  [font=\small]  {$b$};
% Text Node
\draw (202,24.23) node  [font=\small]  {$b$};
% Text Node
\draw (245.19,197.57) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$acc_{l}$};
% Text Node
\draw (201.72,53.33) node  [font=\small,color={rgb, 255:red, 155; green, 155; blue, 155 }  ,opacity=1 ]  {$\mathbf{c}$};
% Text Node
\draw (14.4,52.53) node  [font=\small]  {$\mathbf{c}$};
% Text Node
\draw (14,82.13) node  [font=\small]  {$e$};
% Text Node
\draw (14.1,111.93) node  [font=\small]  {$g$};
% Text Node
\draw (14.4,141.73) node  [font=\small]  {$j$};
% Text Node
\draw (14.5,170.53) node  [font=\small]  {$k$};
% Text Node
\draw (14.1,230.53) node  [font=\small]  {$m$};
% Text Node
\draw (108.4,52.8) node  [font=\small]  {$\mathbf{c}$};
% Text Node
\draw (108,82.4) node  [font=\small]  {$e$};
% Text Node
\draw (108.1,112.2) node  [font=\small]  {$g$};
% Text Node
\draw (108.4,142) node  [font=\small]  {$j$};
% Text Node
\draw (108.5,170.8) node  [font=\small]  {$k$};
% Text Node
\draw (108.1,230.8) node  [font=\small]  {$m$};
% Text Node
\draw (108,260) node  [font=\small]  {$n$};
% Text Node
\draw (202,83.4) node  [font=\small]  {$e$};
% Text Node
\draw (202.1,113.2) node  [font=\small]  {$g$};
% Text Node
\draw (202.4,143) node  [font=\small]  {$j$};
% Text Node
\draw (202.5,171.8) node  [font=\small]  {$k$};
% Text Node
\draw (202,261) node  [font=\small]  {$n$};
% Text Node
\draw (311,82.4) node  [font=\small]  {$e$};
% Text Node
\draw (311.1,112.2) node  [font=\small]  {$g$};
% Text Node
\draw (311.4,142) node  [font=\small]  {$j$};
% Text Node
\draw (311.5,170.8) node  [font=\small]  {$k$};
% Text Node
\draw (311,201) node  [font=\small]  {$\mathbf{l}$};
% Text Node
\draw (311,260) node  [font=\small]  {$n$};
% Text Node
\draw (132.09,226.97) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$una_{n,m}$};
% Text Node
\draw (309.72,53.33) node  [font=\small,color={rgb, 255:red, 155; green, 155; blue, 155 }  ,opacity=1 ]  {$\mathbf{c}$};
% Text Node
\draw (201.72,231.33) node  [font=\small,color={rgb, 255:red, 155; green, 155; blue, 155 }  ,opacity=1 ]  {$m$};
% Text Node
\draw (310.72,231.33) node  [font=\small,color={rgb, 255:red, 155; green, 155; blue, 155 }  ,opacity=1 ]  {$m$};
% Text Node
\draw (309.4,23.63) node  [font=\small]  {$b$};


\end{tikzpicture}


==> fig_exemple_fini.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp32394197299921523] 
\draw  [line width=0.75]  (103.8,200.2) -- (139.6,200.2) -- (139.6,219.54) -- (103.8,219.54) -- cycle ;
%Straight Lines [id:da5103454315814933] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (152.22,89.11) -- (149.6,248.8) ;
%Straight Lines [id:da9625799604219181] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (246.16,86.24) -- (246.8,248.8) ;
%Straight Lines [id:da937826652519754] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (351.56,89.11) -- (350.8,248.4) ;
%Shape: Rectangle [id:dp39055029505322625] 
\draw  [line width=0.75]  (199.09,109.07) -- (234.89,109.07) -- (234.89,128.41) -- (199.09,128.41) -- cycle ;
%Shape: Rectangle [id:dp8416513794122603] 
\draw  [line width=0.75]  (301.69,138.97) -- (337.49,138.97) -- (337.49,158.31) -- (301.69,158.31) -- cycle ;
%Curve Lines [id:da03689428077806867] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (139.93,208.43) .. controls (171.76,232.52) and (195.28,233.43) .. (252.48,180.14) ;
\draw [shift={(253.34,179.33)}, rotate = 136.9] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Shape: Regular Polygon [id:dp0962459706720944] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (281.1,119.83) -- (274.41,131.42) -- (261.03,131.42) -- (254.34,119.83) -- (261.03,108.25) -- (274.41,108.25) -- cycle ;
%Shape: Regular Polygon [id:dp5863365292722718] 
\draw   (93.78,119.03) -- (87.09,130.62) -- (73.71,130.62) -- (67.02,119.03) -- (73.71,107.45) -- (87.09,107.45) -- cycle ;
%Shape: Regular Polygon [id:dp13320010668351145] 
\draw   (92.48,178.53) -- (85.79,190.12) -- (72.41,190.12) -- (65.72,178.53) -- (72.41,166.95) -- (85.79,166.95) -- cycle ;
%Shape: Regular Polygon [id:dp33133807114366276] 
\draw   (187.78,119.3) -- (181.09,130.89) -- (167.71,130.89) -- (161.02,119.3) -- (167.71,107.72) -- (181.09,107.72) -- cycle ;
%Shape: Regular Polygon [id:dp3825724531298007] 
\draw   (186.48,178.8) -- (179.79,190.39) -- (166.41,190.39) -- (159.72,178.8) -- (166.41,167.22) -- (179.79,167.22) -- cycle ;
%Shape: Polygon [id:dp6015095613297166] 
\draw   (186.4,208) -- (179.7,219.54) -- (166.3,219.54) -- (159.6,208) -- (166.3,196.46) -- (179.7,196.46) -- cycle ;
%Shape: Polygon [id:dp15730100429007365] 
\draw   (280.4,209) -- (273.7,220.54) -- (260.3,220.54) -- (253.6,209) -- (260.3,197.46) -- (273.7,197.46) -- cycle ;
%Shape: Polygon [id:dp5246042913035425] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (389.4,149) -- (382.7,160.54) -- (369.3,160.54) -- (362.6,149) -- (369.3,137.46) -- (382.7,137.46) -- cycle ;
%Shape: Polygon [id:dp40275693353577746] 
\draw   (389.4,208) -- (382.7,219.54) -- (369.3,219.54) -- (362.6,208) -- (369.3,196.46) -- (382.7,196.46) -- cycle ;
%Shape: Rectangle [id:dp294546304037402] 
\draw  [line width=0.75]  (198.09,169.57) -- (233.89,169.57) -- (233.89,188.91) -- (198.09,188.91) -- cycle ;
%Shape: Regular Polygon [id:dp6955758409780655] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (280.1,179.33) -- (273.41,190.92) -- (260.03,190.92) -- (253.34,179.33) -- (260.03,167.75) -- (273.41,167.75) -- cycle ;
%Shape: Regular Polygon [id:dp41515587858602165] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (389.1,179.33) -- (382.41,190.92) -- (369.03,190.92) -- (362.34,179.33) -- (369.03,167.75) -- (382.41,167.75) -- cycle ;
%Curve Lines [id:da6369256315030506] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (234.67,120.27) .. controls (248.29,119.59) and (240.21,120.65) .. (252.47,119.94) ;
\draw [shift={(254.34,119.83)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da7931620072938754] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (338.22,149.11) .. controls (351.84,148.43) and (348.06,149.78) .. (360.7,149.11) ;
\draw [shift={(362.6,149)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Straight Lines [id:da3473821810184682] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (447.44,89.4) -- (447.8,248.87) ;
%Straight Lines [id:da28717992359290156] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (552.56,89.18) -- (551.8,248.47) ;
%Shape: Rectangle [id:dp9290672247616546] 
\draw  [line width=0.75]  (400.09,109.14) -- (435.89,109.14) -- (435.89,128.48) -- (400.09,128.48) -- cycle ;
%Shape: Rectangle [id:dp4615386743250496] 
\draw  [line width=0.75]  (502.69,139.04) -- (538.49,139.04) -- (538.49,158.38) -- (502.69,158.38) -- cycle ;
%Shape: Polygon [id:dp869958082377734] 
\draw   (481.4,209.07) -- (474.7,220.6) -- (461.3,220.6) -- (454.6,209.07) -- (461.3,197.53) -- (474.7,197.53) -- cycle ;
%Shape: Polygon [id:dp6933331352914898] 
\draw   (590.4,149.07) -- (583.7,160.6) -- (570.3,160.6) -- (563.6,149.07) -- (570.3,137.53) -- (583.7,137.53) -- cycle ;
%Shape: Polygon [id:dp9983453460104494] 
\draw   (590.4,208.07) -- (583.7,219.6) -- (570.3,219.6) -- (563.6,208.07) -- (570.3,196.53) -- (583.7,196.53) -- cycle ;
%Shape: Rectangle [id:dp4128760078522289] 
\draw  [line width=0.75]  (399.09,169.64) -- (434.89,169.64) -- (434.89,188.98) -- (399.09,188.98) -- cycle ;
%Curve Lines [id:da4468899959406666] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (539.22,149.18) .. controls (552.84,148.5) and (549.06,149.85) .. (561.7,149.18) ;
\draw [shift={(563.6,149.07)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Shape: Regular Polygon [id:dp30327950073583065] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (389.1,119.83) -- (382.41,131.42) -- (369.03,131.42) -- (362.34,119.83) -- (369.03,108.25) -- (382.41,108.25) -- cycle ;
%Shape: Polygon [id:dp7283580755561466] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (480.4,149) -- (473.7,160.54) -- (460.3,160.54) -- (453.6,149) -- (460.3,137.46) -- (473.7,137.46) -- cycle ;
%Curve Lines [id:da5949004056754674] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (233.67,179.77) .. controls (247.29,179.09) and (239.21,180.15) .. (251.47,179.44) ;
\draw [shift={(253.34,179.33)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da5516235060031613] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (139.93,208.43) .. controls (153.55,207.76) and (145.48,208.81) .. (157.73,208.11) ;
\draw [shift={(159.6,208)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da23955876646227958] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (435.89,120.2) .. controls (449.51,119.52) and (441.43,120.58) .. (453.69,119.88) ;
\draw [shift={(455.56,119.77)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da6032022822635317] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (435,179.31) .. controls (448.62,178.63) and (440.55,179.69) .. (452.8,178.99) ;
\draw [shift={(454.67,178.88)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da3442108848849781] 
\draw    (139.74,209.46) .. controls (147.76,188.82) and (175.19,203.39) .. (196.24,181.02) ;
\draw [shift={(197.52,179.6)}, rotate = 130.99] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da48487114474355186] 
\draw    (139.93,208.43) .. controls (141.9,142.11) and (156.43,155.56) .. (197.47,120.91) ;
\draw [shift={(198.72,119.84)}, rotate = 139.4] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da12088282982601495] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (139.93,208.43) .. controls (133.55,96.56) and (192.92,66.7) .. (253.43,119.04) ;
\draw [shift={(254.34,119.83)}, rotate = 221.3] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da02422060535524939] 
\draw    (139.74,209.46) .. controls (139.52,149.25) and (244.98,122.77) .. (299.87,148.64) ;
\draw [shift={(301.52,149.44)}, rotate = 206.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da677163051430355] 
\draw    (233.67,179.77) .. controls (254.8,166.84) and (260.55,159.27) .. (299.71,149.87) ;
\draw [shift={(301.52,149.44)}, rotate = 166.76] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da5228514854183428] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (139.93,208.43) .. controls (132.04,-4.99) and (327.52,129.58) .. (361.18,148.23) ;
\draw [shift={(362.6,149)}, rotate = 207.65] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da6744492753589657] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (233.67,179.77) .. controls (265.5,203.85) and (304.39,203.11) .. (361.74,149.81) ;
\draw [shift={(362.6,149)}, rotate = 136.9] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da20776941667882975] 
\draw    (139.74,209.46) .. controls (118.48,-0.96) and (369.65,87.48) .. (398.59,118.31) ;
\draw [shift={(399.76,119.68)}, rotate = 232.73] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da10570289480424622] 
\draw    (139.93,208.43) .. controls (158.88,239.14) and (242,231.56) .. (309.24,215.44) .. controls (351.54,205.29) and (387.55,191.77) .. (397.35,182.28) ;
\draw [shift={(398.56,180.96)}, rotate = 128.66] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da8429272301754287] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (139.74,209.46) .. controls (153.93,255.29) and (423.29,243.24) .. (454.23,179.84) ;
\draw [shift={(454.67,178.88)}, rotate = 114.05] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da23290031359620267] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (139.93,208.43) .. controls (118.46,-4.12) and (381.83,67.91) .. (454.48,119) ;
\draw [shift={(455.56,119.77)}, rotate = 215.73] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da526458424685257] 
\draw    (139.74,209.46) .. controls (152.5,262.29) and (460.66,249.09) .. (501.56,150.85) ;
\draw [shift={(502.16,149.36)}, rotate = 111.08] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da44056117735269607] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (139.74,209.46) .. controls (134.19,260.22) and (540.07,269.98) .. (563.28,150.87) ;
\draw [shift={(563.6,149.07)}, rotate = 99.13] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da6532223371130883] 
\draw    (233.67,179.77) .. controls (285.4,137.7) and (453.71,190.6) .. (500.77,150.6) ;
\draw [shift={(502.16,149.36)}, rotate = 136.78] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da046773503537721695] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (233.67,179.77) .. controls (262.97,91.32) and (470.23,82.17) .. (562.23,148.07) ;
\draw [shift={(563.6,149.07)}, rotate = 216.27] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da7716944225413247] 
\draw    (435,179.31) .. controls (474.69,165.86) and (490.18,166.96) .. (501.15,150.9) ;
\draw [shift={(502.16,149.36)}, rotate = 121.98] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da6292484131405056] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (435,179.31) .. controls (466.83,203.4) and (505.73,202.66) .. (563.07,149.35) ;
\draw [shift={(563.94,148.54)}, rotate = 136.9] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da08723376672210947] 
\draw    (338.22,149.11) .. controls (359.09,127.87) and (477.45,123.99) .. (500.85,147.86) ;
\draw [shift={(502.16,149.36)}, rotate = 232.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da908211049333919] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (338.22,149.11) .. controls (360.61,68.64) and (472.79,84.56) .. (562.26,148.11) ;
\draw [shift={(563.6,149.07)}, rotate = 215.66] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da3009095877838823] 
\draw    (234.36,179.39) .. controls (253.11,199.74) and (343.49,220.43) .. (397.74,181.55) ;
\draw [shift={(398.56,180.96)}, rotate = 143.77] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da3185352755684201] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (234.36,179.39) .. controls (289.72,204.51) and (374.74,262.06) .. (453.49,180.12) ;
\draw [shift={(454.67,178.88)}, rotate = 133.35] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;

% Text Node
\draw (92.13,244.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$t_{13}$};
% Text Node
\draw (109,206.6) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$enu_{n}$};
% Text Node
\draw (199.09,115.47) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$und_{n,c}$};
% Text Node
\draw (181.67,245.33) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$t_{13} +1$};
% Text Node
\draw (280.8,244.9) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$t_{13} +2$};
% Text Node
\draw (310.19,146.57) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$und_{l}$};
% Text Node
\draw (267.72,120.83) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$\mathbf{c}$};
% Text Node
\draw (80.4,120.03) node  [font=\small]  {$\mathbf{c}$};
% Text Node
\draw (79.1,179.53) node  [font=\small]  {$m$};
% Text Node
\draw (174.4,120.3) node  [font=\small]  {$\mathbf{c}$};
% Text Node
\draw (173.1,179.8) node  [font=\small]  {$m$};
% Text Node
\draw (173,209) node  [font=\small]  {$n$};
% Text Node
\draw (267,210) node  [font=\small]  {$n$};
% Text Node
\draw (376,150) node  [font=\small]  {$\mathbf{l}$};
% Text Node
\draw (376,209) node  [font=\small]  {$n$};
% Text Node
\draw (197.09,175.97) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$und_{n,m}$};
% Text Node
\draw (375.72,120.83) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$\mathbf{c}$};
% Text Node
\draw (266.72,180.33) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$m$};
% Text Node
\draw (375.72,180.33) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$m$};
% Text Node
\draw (400.09,115.54) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$una_{n,c}$};
% Text Node
\draw (382.67,245.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$t_{13} +3$};
% Text Node
\draw (481.8,244.97) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$t_{13} +4$};
% Text Node
\draw (567,243.97) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$t_{14}$};
% Text Node
\draw (511.19,146.64) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$acc_{l}$};
% Text Node
\draw (468.72,120.9) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$\mathbf{c}$};
% Text Node
\draw (468,210.07) node  [font=\small]  {$n$};
% Text Node
\draw (577,150.07) node  [font=\small]  {$\mathbf{l}$};
% Text Node
\draw (577,209.07) node  [font=\small]  {$n$};
% Text Node
\draw (398.09,176.04) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$una_{n,m}$};
% Text Node
\draw (576.72,120.9) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$\mathbf{c}$};
% Text Node
\draw (467.72,180.4) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$m$};
% Text Node
\draw (576.72,180.4) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$m$};
% Text Node
\draw (268,150) node  [font=\small]  {$\mathbf{l}$};
% Text Node
\draw (173,150) node  [font=\small]  {$\mathbf{l}$};
% Text Node
\draw (79.33,150.33) node  [font=\small]  {$\mathbf{l}$};
% Text Node
\draw (467,150) node  [font=\small]  {$\mathbf{l}$};


\end{tikzpicture}

==> fig_exemple_ini.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp32394197299921523] 
\draw  [line width=0.75]  (103.8,200.2) -- (139.6,200.2) -- (139.6,219.54) -- (103.8,219.54) -- cycle ;
%Straight Lines [id:da5103454315814933] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (152.22,89.11) -- (149.6,248.8) ;
%Straight Lines [id:da9625799604219181] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (246.44,89.33) -- (246.8,248.8) ;
%Straight Lines [id:da937826652519754] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (351.56,89.11) -- (350.8,248.4) ;
%Shape: Rectangle [id:dp39055029505322625] 
\draw  [line width=0.75]  (199.09,109.07) -- (234.89,109.07) -- (234.89,128.41) -- (199.09,128.41) -- cycle ;
%Shape: Rectangle [id:dp8416513794122603] 
\draw  [line width=0.75]  (301.69,138.97) -- (337.49,138.97) -- (337.49,158.31) -- (301.69,158.31) -- cycle ;
%Curve Lines [id:da03689428077806867] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (139.93,208.43) .. controls (175.44,232.73) and (219.9,239.86) .. (252.62,209.92) ;
\draw [shift={(253.6,209)}, rotate = 136.62] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Shape: Regular Polygon [id:dp0962459706720944] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (281.1,119.83) -- (274.41,131.42) -- (261.03,131.42) -- (254.34,119.83) -- (261.03,108.25) -- (274.41,108.25) -- cycle ;
%Shape: Regular Polygon [id:dp5863365292722718] 
\draw   (93.78,119.03) -- (87.09,130.62) -- (73.71,130.62) -- (67.02,119.03) -- (73.71,107.45) -- (87.09,107.45) -- cycle ;
%Shape: Regular Polygon [id:dp13320010668351145] 
\draw   (92.48,178.53) -- (85.79,190.12) -- (72.41,190.12) -- (65.72,178.53) -- (72.41,166.95) -- (85.79,166.95) -- cycle ;
%Shape: Regular Polygon [id:dp33133807114366276] 
\draw   (187.78,119.3) -- (181.09,130.89) -- (167.71,130.89) -- (161.02,119.3) -- (167.71,107.72) -- (181.09,107.72) -- cycle ;
%Shape: Regular Polygon [id:dp3825724531298007] 
\draw   (186.48,178.8) -- (179.79,190.39) -- (166.41,190.39) -- (159.72,178.8) -- (166.41,167.22) -- (179.79,167.22) -- cycle ;
%Shape: Polygon [id:dp6015095613297166] 
\draw   (186.4,208) -- (179.7,219.54) -- (166.3,219.54) -- (159.6,208) -- (166.3,196.46) -- (179.7,196.46) -- cycle ;
%Shape: Polygon [id:dp15730100429007365] 
\draw   (280.4,209) -- (273.7,220.54) -- (260.3,220.54) -- (253.6,209) -- (260.3,197.46) -- (273.7,197.46) -- cycle ;
%Shape: Polygon [id:dp5246042913035425] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (389.4,149) -- (382.7,160.54) -- (369.3,160.54) -- (362.6,149) -- (369.3,137.46) -- (382.7,137.46) -- cycle ;
%Shape: Polygon [id:dp40275693353577746] 
\draw   (389.4,208) -- (382.7,219.54) -- (369.3,219.54) -- (362.6,208) -- (369.3,196.46) -- (382.7,196.46) -- cycle ;
%Shape: Rectangle [id:dp294546304037402] 
\draw  [line width=0.75]  (198.09,169.57) -- (233.89,169.57) -- (233.89,188.91) -- (198.09,188.91) -- cycle ;
%Shape: Regular Polygon [id:dp6955758409780655] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (280.1,179.33) -- (273.41,190.92) -- (260.03,190.92) -- (253.34,179.33) -- (260.03,167.75) -- (273.41,167.75) -- cycle ;
%Shape: Regular Polygon [id:dp41515587858602165] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (389.1,179.33) -- (382.41,190.92) -- (369.03,190.92) -- (362.34,179.33) -- (369.03,167.75) -- (382.41,167.75) -- cycle ;
%Curve Lines [id:da07687685155568191] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (139.74,209.46) .. controls (191.33,239.77) and (226.33,236.43) .. (362.6,208) ;
\draw [shift={(362.6,208)}, rotate = 168.21] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da6369256315030506] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (234.67,120.27) .. controls (248.29,119.59) and (240.21,120.65) .. (252.47,119.94) ;
\draw [shift={(254.34,119.83)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da7931620072938754] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (338.22,149.11) .. controls (351.84,148.43) and (348.06,149.78) .. (360.7,149.11) ;
\draw [shift={(362.6,149)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Straight Lines [id:da3473821810184682] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (447.44,89.4) -- (447.8,248.87) ;
%Straight Lines [id:da28717992359290156] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (552.56,89.18) -- (551.8,248.47) ;
%Shape: Rectangle [id:dp9290672247616546] 
\draw  [line width=0.75]  (400.09,109.14) -- (435.89,109.14) -- (435.89,128.48) -- (400.09,128.48) -- cycle ;
%Shape: Rectangle [id:dp4615386743250496] 
\draw  [line width=0.75]  (502.69,139.04) -- (538.49,139.04) -- (538.49,158.38) -- (502.69,158.38) -- cycle ;
%Shape: Polygon [id:dp869958082377734] 
\draw   (481.4,209.07) -- (474.7,220.6) -- (461.3,220.6) -- (454.6,209.07) -- (461.3,197.53) -- (474.7,197.53) -- cycle ;
%Shape: Polygon [id:dp6933331352914898] 
\draw   (590.4,149.07) -- (583.7,160.6) -- (570.3,160.6) -- (563.6,149.07) -- (570.3,137.53) -- (583.7,137.53) -- cycle ;
%Shape: Polygon [id:dp9983453460104494] 
\draw   (590.4,208.07) -- (583.7,219.6) -- (570.3,219.6) -- (563.6,208.07) -- (570.3,196.53) -- (583.7,196.53) -- cycle ;
%Shape: Rectangle [id:dp4128760078522289] 
\draw  [line width=0.75]  (399.09,169.64) -- (434.89,169.64) -- (434.89,188.98) -- (399.09,188.98) -- cycle ;
%Curve Lines [id:da4468899959406666] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (539.22,149.18) .. controls (552.84,148.5) and (549.06,149.85) .. (561.7,149.18) ;
\draw [shift={(563.6,149.07)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Shape: Regular Polygon [id:dp30327950073583065] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (389.1,119.83) -- (382.41,131.42) -- (369.03,131.42) -- (362.34,119.83) -- (369.03,108.25) -- (382.41,108.25) -- cycle ;
%Shape: Polygon [id:dp7283580755561466] 
\draw  [color={rgb, 255:red, 155; green, 155; blue, 155 }  ,draw opacity=1 ] (480.4,149) -- (473.7,160.54) -- (460.3,160.54) -- (453.6,149) -- (460.3,137.46) -- (473.7,137.46) -- cycle ;
%Curve Lines [id:da5949004056754674] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (233.67,179.77) .. controls (247.29,179.09) and (239.21,180.15) .. (251.47,179.44) ;
\draw [shift={(253.34,179.33)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da5516235060031613] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (139.93,208.43) .. controls (153.55,207.76) and (145.48,208.81) .. (157.73,208.11) ;
\draw [shift={(159.6,208)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da23955876646227958] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (435.89,120.2) .. controls (449.51,119.52) and (441.43,120.58) .. (453.69,119.88) ;
\draw [shift={(455.56,119.77)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da6032022822635317] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (435,179.31) .. controls (448.62,178.63) and (440.55,179.69) .. (452.8,178.99) ;
\draw [shift={(454.67,178.88)}, rotate = 176.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da6272466598449091] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (139.74,209.46) .. controls (193.53,247.1) and (318.33,237.5) .. (454.6,209.07) ;
\draw [shift={(454.6,209.07)}, rotate = 168.21] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da8374889471420768] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (139.74,209.46) .. controls (205.68,258.88) and (427.33,236.5) .. (563.6,208.07) ;
\draw [shift={(563.6,208.07)}, rotate = 168.21] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da4275479495021679] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (233.67,179.77) .. controls (274.55,207.4) and (311.81,193.17) .. (360.85,179.74) ;
\draw [shift={(362.34,179.33)}, rotate = 164.78] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da3181389263254073] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (234.67,120.27) .. controls (274.56,148.2) and (311.81,133.68) .. (360.85,120.24) ;
\draw [shift={(362.34,119.83)}, rotate = 164.78] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da33919175500205845] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (435.89,120.2) .. controls (475.78,148.13) and (513.03,133.61) .. (562.07,120.17) ;
\draw [shift={(563.56,119.77)}, rotate = 164.78] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da310794760204927] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (435,179.31) .. controls (474.89,207.24) and (512.14,192.72) .. (561.18,179.28) ;
\draw [shift={(562.67,178.88)}, rotate = 164.78] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;
%Curve Lines [id:da30150454137272376] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (338.22,149.11) .. controls (381.09,176.36) and (403.38,162.82) .. (452.12,149.41) ;
\draw [shift={(453.6,149)}, rotate = 164.78] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (4.37,-1.32) .. controls (2.78,-0.56) and (1.32,-0.12) .. (0,0) .. controls (1.32,0.12) and (2.78,0.56) .. (4.37,1.32)   ;

% Text Node
\draw (92.13,238.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$t_{13}$};
% Text Node
\draw (109,206.6) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$enu_{n}$};
% Text Node
\draw (199.09,115.47) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$und_{n,c}$};
% Text Node
\draw (181.67,239.33) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$t_{13} +1$};
% Text Node
\draw (280.8,238.9) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$t_{13} +2$};
% Text Node
\draw (310.19,146.57) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$und_{l}$};
% Text Node
\draw (267.72,120.83) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$\mathbf{c}$};
% Text Node
\draw (80.4,120.03) node  [font=\small]  {$\mathbf{c}$};
% Text Node
\draw (79.1,179.53) node  [font=\small]  {$m$};
% Text Node
\draw (174.4,120.3) node  [font=\small]  {$\mathbf{c}$};
% Text Node
\draw (173.1,179.8) node  [font=\small]  {$m$};
% Text Node
\draw (173,209) node  [font=\small]  {$n$};
% Text Node
\draw (267,210) node  [font=\small]  {$n$};
% Text Node
\draw (376,150) node  [font=\small]  {$\mathbf{l}$};
% Text Node
\draw (376,209) node  [font=\small]  {$n$};
% Text Node
\draw (197.09,175.97) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$und_{n,m}$};
% Text Node
\draw (375.72,120.83) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$\mathbf{c}$};
% Text Node
\draw (266.72,180.33) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$m$};
% Text Node
\draw (375.72,180.33) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$m$};
% Text Node
\draw (400.09,115.54) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$una_{n,c}$};
% Text Node
\draw (382.67,239.4) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$t_{13} +3$};
% Text Node
\draw (481.8,238.97) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$t_{13} +4$};
% Text Node
\draw (567,237.97) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$t_{14}$};
% Text Node
\draw (511.19,146.64) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$acc_{l}$};
% Text Node
\draw (468.72,120.9) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$\mathbf{c}$};
% Text Node
\draw (468,210.07) node  [font=\small]  {$n$};
% Text Node
\draw (577,150.07) node  [font=\small]  {$\mathbf{l}$};
% Text Node
\draw (577,209.07) node  [font=\small]  {$n$};
% Text Node
\draw (398.09,176.04) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize]  {$una_{n,m}$};
% Text Node
\draw (576.72,120.9) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$\mathbf{c}$};
% Text Node
\draw (467.72,180.4) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$m$};
% Text Node
\draw (576.72,180.4) node  [font=\small,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ]  {$m$};
% Text Node
\draw (268,150) node  [font=\small]  {$\mathbf{l}$};
% Text Node
\draw (173,150) node  [font=\small]  {$\mathbf{l}$};
% Text Node
\draw (79.33,150.33) node  [font=\small]  {$\mathbf{l}$};
% Text Node
\draw (467,150) node  [font=\small]  {$\mathbf{l}$};


\end{tikzpicture}
